Intersection of Parallels as an Early Stopping Criterion

A common way to avoid overfitting in supervised learning is early stopping, where a held-out set is used for iterative evaluation during training to find a sweet spot in the number of training steps that gives maximum generalization. However, such a method requires a disjoint validation set, thus part of the labeled data from the training set is usually left out for this purpose, which is not ideal when training data is scarce. Furthermore, when the training labels are noisy, the performance of the model over a validation set may not be an accurate proxy for generalization. In this paper, we propose a method to spot an early stopping point in the training iterations without the need for a validation set. We first show that in the overparameterized regime the randomly initialized weights of a linear model converge to the same direction during training. Using this result, we propose to train two parallel instances of a linear model, initialized with different random seeds, and use their intersection as a signal to detect overfitting. In order to detect intersection, we use the cosine distance between the weights of the parallel models during training iterations. Noticing that the final layer of a NN is a linear map of pre-last layer activations to output logits, we build on our criterion for linear models and propose an extension to multi-layer networks, using the new notion of counterfactual weights. We conduct experiments on two areas that early stopping has noticeable impact on preventing overfitting of a NN: (i) learning from noisy labels; and (ii) learning to rank in IR. Our experiments on four widely used datasets confirm the effectiveness of our method for generalization. For a wide range of learning rates, our method, called Cosine-Distance Criterion (CDC), leads to better generalization on average than all the methods that we compare against in almost all of the tested cases.

==> sections/figure_tex/04-tbl-sizes.tex <==

\begin{table}[t]
    \caption{Image classification network sizes.}
    \label{tab:experiment:size}
    \setlength{\tabcolsep}{0.6em}
    \begin{tabular}{l l c  c c}
    \toprule
    & &
        \multicolumn{1}{c}{Small} & 
        \multicolumn{1}{c}{Medium} & 
        \multicolumn{1}{c}{Large} \\
        \cmidrule{2-5}
        \multirow{2}{*}{Linear} &
        Layers &
        $[9k, 10]$ & 
        $[25k, 10]$ & 
        $[50k, 10]$ &  \\
        & Params & $90k$&$250k$&$500k$ \\
        \midrule
        \multirow{2}{*}{2-layer MNIST} &
        Layers &
        $[784, 150, 10]$ & 
        $[784, 350, 10]$ & 
        $[784, 700, 10]$ &  \\
        & Params & $119k$ &$250k$&$500k$ \\

        \bottomrule
    \end{tabular}
    \end{table}


==> sections/figure_tex/05-fig-multi.tex <==
\begin{figure*}[t]
    \centering
    \begin{tabular}[]{lccc}

        & \hspace{1.5em}\small a) Layer 1
        & \hspace{1.8em} \small b) Layer 2
        & \hspace{1.2em}\small c) Layer 3
        \\
        \rotatebox[origin=lt]{90}{\hspace{1em} \small Cosine distance}
        &
        \includegraphics[scale=0.33]{sections/figure/multi_L0}
        &
        \includegraphics[scale=0.33]{sections/figure/multi_L1}
        &
        \includegraphics[scale=0.33]{sections/figure/multi_L2}  \\
        & \hspace{1.5em}\small Epochs
        & \hspace{1.8em} \small Epochs
        & \hspace{1.2em}\small Epochs
        
    \end{tabular}
    \caption{Change of direction in different layers of a three-layer network, for different LTR loss functions.}
    \label{fig:multi}
\end{figure*}

==> sections/figure_tex/07-fig-multi_performance.tex <==

\begin{figure*}[t]
    \centering
    \begin{tabular}[]{lcccc}
        & \small RMSE & \small LambdaRank & \small ListNet \\
        \rotatebox[origin=lt]{90}{\hspace{2em} \small NDCG@10}
        &
        \includegraphics[scale=0.33]{sections/figure/performance_yahoo_rmse_5}
        &
        \includegraphics[scale=0.33]{sections/figure/performance_yahoo_lambdaRank_5}
        &
        \includegraphics[scale=0.33]{sections/figure/performance_yahoo_listNet_5}
        &
        \includegraphics[scale=0.4]{sections/figure/performance_legend}  \\
        \rotatebox[origin=lt]{90}{\hspace{2em} \small NDCG@10}
        &
        \includegraphics[scale=0.33]{sections/figure/performance_mslr_rmse_5}
        &
        \includegraphics[scale=0.33]{sections/figure/performance_mslr_lambdaRank_5}
        &
        \includegraphics[scale=0.33]{sections/figure/performance_mslr_listNet_5}  \\
        & \small Learning rate
        & \small Learning rate
        & \small Learning rate
        
    \end{tabular}
    \caption{\emph{\bfseries Three-layer networks.} Performance comparison of \ourmethod with baselines in terms of test NDCG@10 for linear models and different \ac{LTR} loss functions. Top: Yahoo! dataset; Bottom: MSLR dataset.}
    \label{fig:performance_multi}
\end{figure*}


==> sections/figure_tex/07-tbl-mart.tex <==

% LambdaMART
% yahoo 0.7398003199258641
% mslr 0.3887174443659485

\begin{table}[t]
    \caption{Ranking performance in terms of nDCG@10 of \moped linear model with LambdaRank loss and learning rate of $0.01$ with tree-based LambdaMART on the same training data.}
    \label{tab:results:mart}
    \setlength{\tabcolsep}{0.6em}
    \begin{tabular}{l cc  c}
    \toprule
        & \multicolumn{2}{c}{\mOped linear}
        & \multicolumn{1}{c}{Tree-based} \\
        \cmidrule(lr){2-3}\cmidrule(lr){4-4}
        & \ourmethod
        & Oracle
        & LambdaMART \\
        \midrule
        Yahoo! Webscope
        & 0.730 & 0.730 & 0.740\\
        MSLR-WEB30k
        & 0.400 & 0.405& 0.389\\

        \bottomrule
    \end{tabular}
    \end{table}


==> sections/figure_tex/07-tbl-multi_mean.tex <==
 


\begin{table*}[t]
    \caption{\emph{\bfseries Three-layer networks.} Mean and standard deviation of test NDCG@10 for different stopping methods across different train data subsets and different learning rates (Fig.~\ref{fig:performance_multi}).}
    \label{tab:results:mean2}
    \setlength{\tabcolsep}{0.6em}
    \begin{tabular}{l cccccc cccccc}
    \toprule
        & \multicolumn{6}{c}{Yahoo! Webscope}
        & \multicolumn{6}{c}{MSLR-WEB30k}
        \\
        \cmidrule(lr){2-7}\cmidrule(lr){8-13} 
        & \multicolumn{2}{c}{RMSE} & \multicolumn{2}{c}{LambdaRank} & \multicolumn{2}{c}{ListNet}
        & \multicolumn{2}{c}{RMSE} & \multicolumn{2}{c}{LambdaRank} & \multicolumn{2}{c}{ListNet}
        \\
        \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13} 
        & \bf Mean           & \small \bf \textit{STD}
        & \bf Mean           & \small \bf \textit{STD}
        & \bf Mean           & \small \bf \textit{STD}
        & \bf Mean           & \small \bf \textit{STD}
        & \bf Mean           & \small \bf \textit{STD}
        & \bf Mean           & \small \bf \textit{STD}
        \\
        \midrule
        CDC & {\bfseries 0.717} & {\small \itshape 0.0273} & {\bfseries 0.727\rlap{$^*$}} & {\small \itshape \bfseries 0.0054} & {\bfseries 0.727} & {\small \itshape \underline{0.0043}} & {0.352} & {\small \itshape 0.0345} & {\bfseries 0.392\rlap{$^*$}} & {\small \itshape \bfseries 0.0220} & {\underline{0.385}} & {\small \itshape \underline{0.0206}}  \\
        CV & {0.707} & {\small \itshape 0.0271} & {0.713} & {\small \itshape 0.0142} & {0.714} & {\small \itshape 0.0149} & {\bfseries 0.373} & {\small \itshape \underline{0.0299}} & {0.358} & {\small \itshape 0.0442} & {0.366} & {\small \itshape 0.0369}  \\
        EB & {\underline{0.710}} & {\small \itshape 0.0249} & {\underline{0.723}} & {\small \itshape 0.0119} & {\underline{0.727}} & {\small \itshape \bfseries 0.0042} & {0.363} & {\small \itshape \bfseries 0.0198} & {\underline{0.366}} & {\small \itshape 0.0577} & {\bfseries 0.388} & {\small \itshape \bfseries 0.0190}  \\
        GD & {0.706} & {\small \itshape \bfseries 0.0136} & {0.720} & {\small \itshape 0.0113} & {0.712} & {\small \itshape 0.0167} & {0.359} & {\small \itshape 0.0322} & {0.356} & {\small \itshape 0.0345} & {0.349} & {\small \itshape 0.0396}  \\
        Fixed & {0.692} & {\small \itshape \underline{0.0193}} & {0.698} & {\small \itshape \underline{0.0111}} & {0.701} & {\small \itshape 0.0142} & {\underline{0.366}} & {\small \itshape 0.0314} & {0.332} & {\small \itshape \underline{0.0233}} & {0.352} & {\small \itshape 0.0400}  \\
        \midrule
        Oracle & {0.727} & {\small \itshape 0.0050} & {0.731} & {\small \itshape 0.0044} & {0.730} & {\small \itshape 0.0030} & {0.399} & {\small \itshape 0.0126} & {0.406} & {\small \itshape 0.0096} & {0.396} & {\small \itshape 0.0145}  \\

        \bottomrule
    \end{tabular}
    \end{table*}


    

==> sections/figure_tex/alpha.tex <==
\begin{figure}[t]
    \centering
    \begin{tabular}{lc}

        \rotatebox[origin=lt]{90}{\hspace{0.1em} \small Cosine distance}
        &
        \includegraphics[scale=0.27]{sections/figure/cosine_to_pinv} \\
        & \hspace{-7em} \small Epochs
        
    \end{tabular}
    \caption{Cosine distance of weights with the minimum-$\ell_2$ solution by Moore-Penrose inverse for different \ac{LTR} loss functions.}
    \label{fig:alpha}
\end{figure}


==> sections/figure_tex/euc_convergence.tex <==
\begin{figure}[t]
    \centering
    \begin{tabular}[]{lcc}

        \rotatebox[origin=lt]{90}{\hspace{-0.4em} \small Euclidean distance}
        &
        \includegraphics[scale=0.27]{sections/figure/l2distances}  \\
        & \small Epochs
        
    \end{tabular}
    \caption{Convergence of the magnitude of randomly initialized weight vectors of two models with the same (left) and different (right) \ac{LTR} loss function.}
    \label{fig:eucconvergence}
\end{figure}

% \begin{figure}[t]
%     \centering
%     \label{fig:nonconvergence}
%     \begin{tabular}[]{lc}

%         \rotatebox[origin=lt]{90}{\hspace{3em} \small Cosine distance}
%         &
%         \includegraphics[scale=0.5]{sections/figure/nonconvergence} \\
%         & \small Epochs
        
%     \end{tabular}
%     \caption{Convergence of randomly initialized parameter vectors for different \ac{LTR} loss functions.}
% \end{figure}

% \begin{figure}
%     \centering
%     \subfloat[Epochs]{
%     \includegraphics[width=0.5\columnwidth]{sections/figure/convergence}\label{fig:convergence}
%     }
%     \subfloat[Epochs]{
%     \includegraphics[width=0.5\columnwidth]{sections/figure/nonconvergence}\label{fig:nonconvergence}
%     }
%     \caption{Convergence of randomly initialized parameter vectors for (a) the same; and (b) different \ac{LTR} loss functions.}
%         % \label{fig:per_user}
% \end{figure}

==> sections/figure_tex/self.tex <==
\begin{figure}[t]
    \centering
    \begin{tabular}{lcc}

        \rotatebox[origin=lt]{90}{\hspace{0.1em} \small Cosine distance}
        &
        \includegraphics[scale=0.27]{sections/figure/self} &
        \includegraphics[scale=0.27]{sections/figure/self2} \\
        & \small Epochs
        & \small Epochs
        
    \end{tabular}
    \caption{Cosine distance of weights with their initial values for different \ac{LTR} loss functions.
    The plots correspond to two different random initializations.
    Horizontal dotted lines indicate the threshold of $0.01$ for the cosine distance of two models (Fig.~\ref{fig:convergence}-a).}
    \label{fig:self}
\end{figure}


==> sections/figure_tex/sensitivity.tex <==
\begin{figure*}[t]
    \centering
    \begin{tabular}[]{lcccc}
        & \small RMSE & \small LambdaRank & \small ListNet \\
        \rotatebox[origin=lt]{90}{\hspace{2em} \small NDCG@10}
        &
        \includegraphics[scale=0.35]{sections/figure/sensitivity_yahoo_rmse}
        &
        \includegraphics[scale=0.35]{sections/figure/sensitivity_yahoo_lambdaRank}
        &
        \includegraphics[scale=0.35]{sections/figure/sensitivity_yahoo_listNet}
        &
        \includegraphics[scale=0.4]{sections/figure/sensitivity_legend}  
        \\
        \rotatebox[origin=lt]{90}{\hspace{2em} \small NDCG@10}
        &
        \includegraphics[scale=0.35]{sections/figure/sensitivity_mslr_rmse}
        &
        \includegraphics[scale=0.35]{sections/figure/sensitivity_mslr_lambdaRank}
        &
        \includegraphics[scale=0.35]{sections/figure/sensitivity_mslr_listNet}  \\
        & \small Threshold ($\theta$)
        & \small Threshold ($\theta$)
        & \small Threshold ($\theta$)
        
    \end{tabular}
    \caption{Sensitivity of \ourmethod with respect to the threshold ($\theta$) for different \ac{LTR} loss functions. Top: Yahoo! dataset; {Bottom: MSLR dataset.}}
    \label{fig:sensitivity}
\end{figure*}

\begin{figure}[t]
    \centering
    \begin{tabular}{lc}

        \rotatebox[origin=lt]{90}{\hspace{0.1em} \small Cosine distance}
        &
        \includegraphics[scale=0.27]{sections/figure/convergence_bars} \\
        & \hspace{-7em} \small Epochs
        
    \end{tabular}
    \caption{Stopping epoch ranges corresponding to threshold range of $\theta\in [0.1, 0.15]$ for different \ac{LTR} loss functions.}
    \label{fig:bar}
\end{figure}


==> sections/figure_tex/small.tex <==
\begin{figure*}[t]
    \centering
    \begin{tabular}[]{lcccc}
        & \small RMSE & \small LambdaRank & \small ListNet \\
        \rotatebox[origin=lt]{90}{\hspace{2em} \small NDCG@10}
        &
        \includegraphics[scale=0.33]{sections/figure/performance_small_yahoo_rmse}
        &
        \includegraphics[scale=0.33]{sections/figure/performance_small_yahoo_lambdaRank}
        &
        \includegraphics[scale=0.33]{sections/figure/performance_small_yahoo_listNet}
        &
        \includegraphics[scale=0.4]{sections/figure/performance_legend}  \\
        % \rotatebox[origin=lt]{90}{\hspace{2em} \small NDCG@10}
        % &
        % \includegraphics[scale=0.33]{sections/figure/performance_small_mslr_rmse}
        % &
        % \includegraphics[scale=0.33]{sections/figure/performance_small_mslr_lambdaRank}
        % &
        % \includegraphics[scale=0.33]{sections/figure/performance_small_mslr_listNet}  \\
        & \small Learning rate
        & \small Learning rate
        & \small Learning rate
        
    \end{tabular}
    \caption{Performance comparison of \ourmethod with baselines with extremely low volumes of training data in terms of test NDCG@10.}
    \label{fig:performance_small}
\end{figure*}


==> sections/figure_tex/underparameterized.tex <==
\begin{figure*}[t]
    \centering
    \begin{tabular}[]{lcccc}
        & RMSE & LambdaRank & ListNet \\
        \rotatebox[origin=lt]{90}{\hspace{2em} \small NDCG@10}
        &
        \includegraphics[width=0.5\columnwidth]{sections/figure/performance_under_yahoo_rmse}
        &
        \includegraphics[width=0.5\columnwidth]{sections/figure/performance_under_yahoo_lambdaRank}
        &
        \includegraphics[width=0.5\columnwidth]{sections/figure/performance_under_yahoo_listNet}
        &
        \includegraphics[width=0.25\columnwidth]{sections/figure/performance_legend}  \\
        % \rotatebox[origin=lt]{90}{\hspace{2em} \small NDCG@10}
        % &
        % \includegraphics[width=0.5\columnwidth]{sections/figure/performance_under_mslr_rmse}
        % &
        % \includegraphics[width=0.5\columnwidth]{sections/figure/performance_under_mslr_lambdaRank}
        % &
        % \includegraphics[width=0.5\columnwidth]{sections/figure/performance_under_mslr_listNet}  \\
        & \small Learning rate
        & \small Learning rate
        & \small Learning rate
        
    \end{tabular}
    \caption{Performance comparison of \ourmethod with baselines with very low training data in terms of test NDCG@10 for different \ac{LTR} loss functions. Top: Yahoo! dataset; Bottom: MSLR dataset.}
    \label{fig:performance_under}
\end{figure*}

